On-Device Machine Learning: An Algorithms and Learning Theory Perspective

The predominant paradigm for using machine learning models on a device is to train a model in the cloud and perform inference using the trained model on the device. However, with increasing number of smart devices and improved hardware, there is interest in performing model training on the device. Given this surge in interest, a comprehensive survey of the field from a device-agnostic perspective sets the stage for both understanding the state-of-the-art and for identifying open challenges and future avenues of research. However, on-device learning is an expansive field with connections to a large number of related topics in AI and machine learning (including online learning, model adaptation, one/few-shot learning, etc.). Hence, covering such a large number of topics in a single survey is impractical. This survey finds a middle ground by reformulating the problem of on-device learning as resource constrained learning where the resources are compute and memory. This reformulation allows tools, techniques, and algorithms from a wide variety of research areas to be compared equitably. In addition to summarizing the state-of-the-art, the survey also identifies a number of challenges and next steps for both the algorithmic and theoretical aspects of on-device learning.

==> Systems.tex <==
% !TEX root = OnDevice.tex

% backlog

%In view of this, there has been a few work which proposes a fused multiply-add chip architectures \cite{bruguera2005floating,quinnell2007floating}

%A state-of-the-art deep neural network model often has couple millions of parameters, thus the majority of memory is occupied by the model weights and its intermediate feature representation fo the input data \cite{lu2017modeling}.    ??? What is the message???

To successfully design an on-device machine learning model meeting the resource requirements for speed, memory, and energy, it requires a complete view of the hardware system, software framework, and model formulation. In this section, we first review the advances in hardware optimization in \autoref{sec:hardware_optimization} and then survey the existing software frameworks and tools for the edge in \autoref{sec:software_optimization}. Note that there are a few research directions that adopt a mathematical modeling approach for system optimization. Such approaches are later covered in  \autoref{sec:efficienttraining}.

%We leave the solution for mathematical modeling in \highlight{\autoref{sec:efficienttraining}}.

Any \acs{ML}-based application has two important operational phases, training and inference. Generally, training is more resource intensive requiring a large labeled dataset and significant computational resources. %, especially when gradient-based optimization is used.
Depending on the scale of the application, available data, and hardware constraints; the training process can even take multiple days to finish. %This in turn requiring access to large computation and energy resources.
This level of resource-utilization is obviously unsuited for edge devices with limited resource availability. Inference, on the other hand, has a lower resource footprint. Although there are quantitative differences in the resource requirements during training vs. inference phase, a vast majority of the systems research view these phases in similar light and target system optimizations applicable to both training/inference phase. But given this obvious utilization differential, we provide a brief summary of the unique challenges faced by the training process in \autoref{sec:unique_challenges_in_training}.

%problem of resource constraints is further compounded when attempting to train on an edge device due to the hardware constraints.
  
%has more relaxed hardware requirements since the model only has to execute the forward pass algorithm without the gradient updates.
 

%The hardware requirements still depend on both the scale of the model and number and dimensions of input data, but with hardware optimization scalable inference is reasonably fast, even on edge devices. It is for such reasons that many computer vision applications such as predictions of traffic pattern and store wait times can be deployed on edge devices. Similarly, applications running on autonomous vehicles and drone and robot navigation can provide for fast inference on device without relying on latency or security risks of cloud based computation and communication. Hence research based on hardware optimization for learning could provide for similar advantages.

\subsection{Hardware Optimization}\label{sec:hardware_optimization}
This section provides a brief summary of hardware optimization research targeted for resource constrained applications. A more comprehensive survey is available in \cite{sze2017efficient}.
%In this section, we briefly surveyed the techniques to alleviates the resource constraints mentioned in \autoref{sec:resource_constraints}.  For more detailed discussion, we refer the readers to a more comprehensive survey \cite{sze2017efficient}.

\subsubsection{Processor}

The computational speed of \ac{ML} models is driven by the number of mathematical operations and the processing speed of the hardware.
From the hardware perspective, increasing the number of operations/instruction per second of the processor is a crucial step to improving the system performance. Different hardware architectures and designs have been proposed and developed to accelerate this computation.

Increasing the clock frequency results in more \ac{IPS} and has been successfully used to directly boost the processing speed in the past decades. However, it is no longer effective as the Dennard's scaling law has broken down due to the current leakage and resulting heat problems \cite{bohr200730}. The inability to increase clock frequency has forced people to invest in the architecture design of processors, especially in parallelizing operations.

%Depending on the structure of machine learning model and size and dimensions of datapoints, different hardware architectures could be utilized to provide computation gains.
These parallel architectures fall into two major categories, spatial and temporal. The temporal architectures allow vectorizations (i.e. \ac{SIMD}), parallel processing threads (i.e. \ac{SIMT}) among other techniques using a centralized control structure with magnitudes of \acp{ALU}. The \acp{ALU} perform data communication (read/write) to and from the memory hierarchy and do not interact with one another. All the \acp{ALU} are controlled by the same controller and utilize the same memory (register file). This is an efficient approach for intensive computations when the {\bf same} operation needs to be applied repeatedly.  On the other hand, spatial architectures allow \acp{ALU} to process the data as well as communicate with each other directly. They can have their own control logic and local memory (individual register files) and can behave as a discrete \ac{PE}.  These additional components provide more versatile processing ability than the temporal architecture. Temporal architectures are deployed in CPUs and GPUs, while ASIC- and FPGA-based designs are common for spatial architecture implementations.

Linear algebra, the foundation of most \ac{ML} algorithms, relies on \ac{MAC} operations. Since \ac{MAC} operations are easy to parallelize, many high-performance hardware architectures have been developed to allow for fast and efficient parallelized computations, and both spatial and temporal architectures can be exploited in conjunction. Depending on the structure of the machine learning model, and size and dimensions of the data, different hardware architectures should be analyzed and utilized for the best computation gains, along with the tuning of algorithm implementation (e.g. \cite{lahabar2009singular,xu2018deep}).

\subsubsection{Memory}

The available device memory limits the overall model complexity and data size that can be processed at any given time.  Given that the specification choices for memory are limited, current research efforts focus on either speed-memory tradeoff or model complexity reductions from an algorithm perspective.  We revisit such approaches in \autoref{subsec:reducemodelcomplexity}.

Another important research topic is targeted towards striking a balance between data access to off-chip memory vs. the cache memory of the processor. For most machine learning algorithms a typical \ac{MAC} operation requires memory reads for obtaining the algorithm's state variables (like filter weight, filter map activation, partial sum etc.) and a memory write for the state updates. Maintaining the state variables and optimizing the data-flow between the cache vs. off-chip memory is crucial for fast execution. For processors like CPU and GPU, these optimizations are handled in several software libraries, like OpenBLAS, Intel MKL, cuDNN, etc., which are discussed later in \autoref{sec:software_optimization}.  For accelerators using spatial architecture, many approaches have been proposed, especially for \ac{DNN} models to exploit the reuse of convolutional, feature map, and filter parameters. Some of the approaches could also be extended to other algorithms and models. The approaches can be broadly grouped as, 
\begin{itemize}
    \item \ac{WS} data-flow maximizes the access of weights already in a register file of the \ac{PE}. This is a greedy approach that processes as many \ac{MAC} operations that use the same weights, while inputs and partial sums are offloaded to the spatial buffer(see \cite{sankaradas2009massively,sriram2010towards,chakradhar2010dynamically,park2015a,cavigelli2017origami} ). 
    \item \ac{OS} data-flows optimize the constant updates to partial sums by streaming the input activations and broadcasting the weights to all \acp{PE} in the spatial array (see \cite{gupta2015deep,du2015shidiannao,peemen2013memory}).
    \item \ac{NLR} tries to increase global storage buffer capacity by removing all storage memory allocated to \acp{PE}. This leads to an increase in traffic among \acp{PE} themselves as well as the buffer but can provide high energy gains for specific models like convolution filter weights and their resulting partial sums (see \cite{zhang2015optimizing,chen2014dadiannao})
    \item \ac{RS} data-flows allow efficiency in the memory register of \acp{PE} by keeping 1-D rows of matrices (like 2D convolution matrix) stationary and streaming the input activations in a sliding window fashion while allowing the other \acp{PE} to compute partial sums iteratively (see \cite{chen2017eyeriss}).
\end{itemize}

In addition, off-chip memory access also consumes orders-of-magnitude more energy compared to the in-chip cache access \cite{horowitz2014computing}. Thus, the improvement on the data-flow model also results in a significant reduction of energy consumption. 

%\ac{WS} \cite{sankaradas2009massively,sriram2010towards,chakradhar2010dynamically,park2015a,cavigelli2017origami},  \ac{OS} \cite{gupta2015deep,du2015shidiannao,peemen2013memory}, \ac{NLR} \cite{zhang2015optimizing,chen2014dadiannao} and  \ac{RS} \cite{chen2017eyeriss}. %\highlight{[96] check with Samarth on reference}. 


%\ac{WS} dataflow maximizes the access of weights already in a register file of the \ac{PE}, processing as many \ac{MAC} operations that use the same weights greedily, while inputs and partial sums are offloaded to the spatial buffer. \ac{OS} dataflows optimize the constant updates to partial sums by streaming the input activations and broadcasting the weights to all \acp{PE} in the spatial array. \ac{NLR} tries to increase global storage buffer capacity, by removing all storage memory allocated to \acp{PE}. This leads to an increase in traffic among \acp{PE} themselves as well as the buffer but can provide high energy gains for specific models like Convolution filter weights and their resulting partial sums. \ac{RS} flows allow efficiency in the memory register of \acp{PE} by keeping 1-D rows of matrices (like 2D convolution matrix) stationary and streaming the input activations in a sliding window fashion while allowing the other \acp{PE} to compute partial sums iteratively.



% talk memory
%For a given model with a fixed input size, the major variance of memory footprint comes from the intermediate data. As commonly optimized for the computing performance, the memory is preallocated for variables without releasing them after each use. However, the memory space recycling can significantly reduce the memory usage with a cost of designing the "inplace" and "co-share" strategies \cite{chen2015mxnet}. With a fixed model and memory allocation strategy, the memory footprint is proportional to the float representation.  

\subsubsection{Energy}
% talk energy
Energy efficiency of a model is another important constraint for edge devices. To optimize energy consumption, processors typically based on spatial architectures allow speedups by providing a memory hierarchy for low-cost data access. Their general structure as mentioned above uses a global buffer to connect the \ac{DRAM} with the \ac{PE} network which allows for data communication between the \acp{ALU} using their individual register files. The data flows can then be designed to exploit the memory read operations for cumulative reuse. The strategy could also use the model’s inherent structure for a more tailored data flow, allowing for adaptive hierarchies during different stages of model processing. Refer to \cite{sze2017efficient} for detailed discussion.


In addition to the fetching data from memory, recent developments have integrated memory with computation. Compared with accessing \ac{DRAM} data, running \ac{MAC} operations in memory has lead to 12 times more energy savings \cite{zhang2016machine}. And pre-processing data at the analog stage can reduce the number of conversions and data movement by an order of magnitude \cite{likamwa2016redeye,wang2012180nm}.  This area is still an active research topic with the potential to reduce energy consumption from different aspects.

Overall the focus on designing better and more robust hardware paradigms has resulted in powerful hardware such as the Intel’s Xeon Phi processors with increased focus on vectorized instructions for Deep learning \cite{sodani2016knights}, Nvidia’s PASCAL GP100 GPU which allow of 16-b floating-point (FP16) MAC operations on a single precision core \cite{nvidia2016nvidia}, along with embedded System-on-Chips (SoCs) as Nvidia Tegra and Samsung Exynos allow for inference on edge devices \cite{ditty2014nvidia,prakash2015energy}. Though hardware designs for optimized and parallel data processing have allowed for fast and high performance, their constraints are still prohibitive to allow training on edge devices in the current stage. Hence this invites more focus on the algorithmic aspects of large scale \ac{DNN} training.

\subsection{Software \& System Library Optimization}\label{sec:software_optimization}

Another alternative approach towards building resource efficient AI applications is directed towards designing optimized software libraries catered towards the underlying hardware. Most often, such specialized software implementations handle efficient matrix multiplications. For example,  OpenBLAS, Intel MKL, etc. for CPUs ,  and cuBLAS, cuDNN, etc. for GPUs. Matrix multiplications generally form the building block of most operations in a machine learning algorithm and are also typically the most time-consuming. Lately, with the emergence of deep-learning, convolution operations (extensively used in vision-related tasks) and the underlying matrix multiplication have been specifically targeted for optimization. In some studies the matrix multiplications use a relaxed form of the Toeplitz matrix, to reduce the computational load at the cost of an increased memory access load. Winograd’s  algorithm \cite{lavin2016fast} which transforms the feature and filter maps, and Strassen’s Algorithm \cite{cong2014minimizing},  which reduces computations in a matrix multiplication from $O(N^3)$ to $O(N^{2.807})$ both allow for reductions in computational complexity, and present interesting directions for future research. Techniques such as \acp{FFT} \cite{mathieu2013fast,dubout2012exact} can reduce number of multiplications from ($N_o^2 * N_f^2$) to ($N_o^2 \times \log_2N_o$), where the output size is $N_o\times N_o$ and the filter size is $N_f \times N_f$. More optimizations can be performed on \acp{FFT} to reduce the number of operations such as precomputing the \ac{FFT} of the filters, breaking the input feature maps into various channels after a single initial computation, and transformation algorithms on symmetric Fourier transforms. All the above algorithms have different efficiencies depending on the shape of the convolution operations. In practice, the best algorithm is  dynamically chosen by the libraries (e.g. MKL and cuDNN) \cite{sze2017efficient} based on the problem at hand.

Besides using the libraries directly, there are software frameworks and toolboxes which directly optimizes the machine learning model to be deployed to the specific edge device. For instance, the Intel Distribution of OpenVINO toolkit optimizes \ac{CNN}-based deep learning inference at heterogeneous devices by Intel (i.e. CPU, GPU, Movidius VPU, and FPGA) \cite{intel2019openvino}.  Apple's Core ML helps data scientists to directly convert \ac{ML} models and optimizes them for Apple devices \cite{apple2019coreml}. Similarly, Tensorflow Lite from Google,  {\it ncnn} from Tencent are optimized more for the \ac{DNN} models for mobile and embedded systems (i.e. Raspberry Pi) \cite{google2019tensorflowlite,tencent2019ncnn}.
Note however, all these existing frameworks only support model inference rather than on-device model training.

\subsection{Unique Challenges in Training}\label{sec:unique_challenges_in_training}


%\highlight{--jason comment-- there are some challenges for training specifically. They might be rearranged to other places.  So I keep them as bullet points and will enrich them once the overall paper is in shape}

%\highlight{Temp paragraph will decide the scope and placement later}

%\begin{enumerate}
%    \item long runtime of training
%    \item Storage of training data
%   \item stability of training
%\end{enumerate}

Recent progress in model compression, especially in \ac{DNN} models, has enabled many applications on edge devices. However, all but few are for the inference stage. Below, we highlight the unique challenges of the training process and their implications on the system aspect.
First, training typically requires more data than the inference process. Besides, the advance in the algorithm design, it occasionally needs additional storage space for the training data. Second, the computation requirement is higher for training and results in more time and energy consumption than the inference only applications. Third, the training process often relies on additional variables and thus the memory footprint is also higher than inference alone.

%Given the complexities of the system infrastructure and software optimization, it is non-trivial to compute or even model the runtime, memory footprint, and energy consumption.  We discuss the modeling efforts in \ref{subsec:resourcemodeling}.

==> abstract.tex <==
Abstract
